Accelerating Sparse DNN Models without Hardware-Support via Tile-Wise Sparsity

Network pruning can reduce the high computation cost of deep neural network (DNN) models. However, to maintain their accuracies, sparse models often carry randomly-distributed weights, leading to irregular computations. Consequently, sparse models cannot achieve meaningful speedup on commodity hardware (e.g., GPU) built for dense matrix computations. As such, prior works usually modify or design completely new sparsity-optimized architectures for exploiting sparsity. We propose an algorithm-software co-designed pruning method that achieves latency speedups on existing dense architectures. Our work builds upon the insight that the matrix multiplication generally breaks the large matrix into multiple smaller tiles for parallel execution. We propose a tiling-friendly "tile-wise" sparsity pattern, which maintains a regular pattern at the tile level for efficient execution but allows for irregular, arbitrary pruning at the global scale to maintain the high accuracy. We implement and evaluate the sparsity pattern on GPU tensor core, achieving a 1.95x speedup over the dense model.

==> tex/methodology.tex <==
\section{methodology} \label{sec:methodology}
\subsection{Cutalss}
\subsection{Optimization for BERT (Transpose, Kernel fusion)}
\subsection{Tricks on pruning (multi-stages, ...)}
\subsubsection{multi-stages}
Our implementation is based on the hierarchically blocked structuresCUTLASS\cite{cutlass2019} for GEMM. 
Compared to pruning lots of weights in one time, and fine tune with many epoches, we find that the performance of pruning few weights time by time and fine tune few epoches will be better. For example, if the final sparsity is 40\%, the accuracy of pruning 40\% weights and fine-tuning three epoches is 82.12\%, but the accuracy of pruning 20\% weights in first time and prune 10\% weight in other times and fine-tuning one epoch after each pruning is 82.52\%. 

\subsubsection{Consider whole network v.s. consider layer by layer}

Different pruning region for each time is also leads to different performance. If we compute the scores of all layers, and prune the lower score weights on whole network, the accuracy would be better. But the reduction of FLOP would be worse. For example, if we prune 50\% on both K and N dimension, the ideal FLOP reduction ratio is 75\%. But the real reduction ratio in our experiment is about 69\%. On the other hand, if we compute the score and prune the lower score weights layer by layer, then the FLOP reduction ratio will be 75\% as we expect, but the accuracy would be worse. 


